Disentangled Multi-Fidelity Deep Bayesian Active Learning

To balance quality and cost, various domain areas of science and engineering run simulations at multiple levels of sophistication. Multi-fidelity active learning aims to learn a direct mapping from input parameters to simulation outputs at the highest fidelity by actively acquiring data from multiple fidelity levels. However, existing approaches based on Gaussian processes are hardly scalable to high-dimensional data. Deep learning-based methods often impose a hierarchical structure in hidden representations, which only supports passing information from low-fidelity to high-fidelity. These approaches can lead to the undesirable propagation of errors from low-fidelity representations to high-fidelity ones. We propose a novel framework called Disentangled Multi-fidelity Deep Bayesian Active Learning (D-MFDAL), which learns the surrogate models conditioned on the distribution of functions at multiple fidelities. On benchmark tasks of learning deep surrogates of partial differential equations including heat equation, Poisson's equation and fluid simulations, our approach significantly outperforms state-of-the-art in prediction accuracy and sample efficiency.

==> def.tex <==
%\usepackage{iclr2021_conference,times}

% Optional math commands from https://github.com/goodfeli/dlbook_notation.
\input{math_commands.tex}

\usepackage{url}

\usepackage{microtype}
\usepackage{graphicx}
\usepackage{booktabs} %
\usepackage{pifont}
%
%
%
%
\usepackage{hyperref}

%
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

%
% \usepackage{icml2020}

%
\usepackage{caption}
%
%
%
\usepackage{natbib}

%
%
%
%
%
%
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\let\Bbbk\relax
%\usepackage{fullpage}

\usepackage{xcolor}
%
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage{hyperref}
\usepackage{bm}
\usepackage{nicefrac}
%
\usepackage{wrapfig}
\usepackage{lipsum}

%
%
%
\usepackage{algorithm,algorithmic}
\usepackage[linesnumbered, ruled,vlined,algo2e]{algorithm2e}

%


%
%
%
\newcommand{\alg}{Rob-ULA\xspace}
\newcommand{\N}{\mathcal N}

\newcounter{assumption}%
\renewcommand{\theassumption}{\arabic{assumption}}

\newenvironment{assumption}[1][]{\begin{trivlist}\item[] \refstepcounter{assumption}%
 {\bf{Assumption\ \theassumption\ }}{(#1)}.  }{%
 \ifvmode\smallskip\fi\end{trivlist}}

%

%
%
\newcommand{\acc}{\varepsilon_{\textsf{acc}}}
% \newcommand{\rd}{\mathrm{d}}
\newcommand{\ssh}{\widehat{h}}
\newcommand{\lmx}{\lambda_{\text{max}}}
\newcommand{\lmn}{\lambda_{\text{min}}}
\newcommand{\eup}{\bar{\epsilon}}
\newcommand{\elo}{\underline{\epsilon}}
\newcommand\ip[2]{\langle #1, #2 \rangle}
\newcommand{\wtS}{\widetilde{\Sigma}}
\newcommand{\ex}{\mathbb{E}}
\newcommand{\lip}{\widehat{L}}
\newcommand{\conv}{\widehat{m}}
\newcommand{\cond}{\kappa}
\newcommand{\covsc}{\beta}
\newcommand{\wass}{\text{W}_2}
\newcommand{\convav}{\bar{\conv}}
\newcommand{\lipav}{\bar{\lip}}
\newcommand{\pari}{\tilde{\param}}
%
%
\newcommand{\pot}{U}
\newcommand{\tpot}{\tilde{U}}
\newcommand{\hpot}{\widehat{U}}

\newcommand{\density}{p}
\newcommand{\initial}{p^0}
\newcommand{\target}{\ensuremath{p^*}}

\newcommand{\brackets}[1]{\left[ #1 \right]}
\newcommand{\parenth}[1]{\left( #1 \right)}
\newcommand{\bigparenth}[1]{\big( #1 \big)}
\newcommand{\biggparenth}[1]{\bigg( #1 \bigg)}
\newcommand{\braces}[1]{\left\{ #1 \right \}}
\newcommand{\abss}[1]{\left| #1 \right |}
\newcommand{\angles}[1]{\left\langle #1 \right \rangle}
\newcommand{\tp}{^\top}

\def\vx{{\bf x}}
\def\vX{{\bf X}}
\def\vy{{\bf y}}
\def\vz{{\bf z}}
\def\vv{{\bf v}}
\def\mD{{\rm D}}
\def\mQ{{\rm Q}}
\def\rd{\mathrm{d}}
\def\rT{{\rm T}}
\def\ball{\mathbb{B}}
\def\mI{\mathrm{I}}
\def\lX{\mathcal{X}}
\def\lY{\mathcal{Y}}

\def\normal{\mathcal{N}}
\newcommand{\thetastar}{\theta_*}
\newcommand*{\p}{p}
\newcommand*{\q}{\mathbf{q}}
\newcommand*{\pmu}{\boldsymbol{\mu}}
\def\mI{\mathrm{I}}
%
%
%
%
%
%
%
%


\newcommand*\Mirr[1]{\textsc{Mirr} (#1)}
\newcommand*\Wd[0]{\textit{W}_2}
\newcommand*\dd[2]{\frac{\partial #1}{\partial #2}}
\newcommand*\stein[1]{\mathcal{A}_{#1}}
\newcommand*\w[0]{\textbf{w}}
\newcommand*\at[2]{\left.#1\right|_{#2}}
\newcommand*\ps[0]{p^*}
\newcommand*\del[0]{\partial}
% \newcommand*\R[0]{\mathbb{R}}
\newcommand*\Z[0]{\mathbb{Z}}
\renewcommand*\div[0]{\nabla \cdot}
\newcommand*\ddt[0]{\frac{d}{d t}}
\newcommand*\dds[0]{\frac{d}{d s}}
\newcommand*\ddp[1]{\frac{\delta #1}{\delta p}}
\newcommand*\tr[0]{\text{tr}}
\newcommand*\kl[2]{\text{KL}\left(#1\|#2\right)}
% \newcommand{\KL}[2]{\mathrm{KL}\left(#1~\Vert~ #2\right)}
\newcommand*\lin[1]{\left\langle #1\right\rangle}
\newcommand*\E[1]{\mathbb{E}\left[#1\right]}
\newcommand*\Ep[2]{\mathbb{E}_{#1}\left[#2\right]}
%
\newcommand*\slope[1]{\|\mathcal{D}_{#1}\|}
\newcommand*\md[1]{\|\frac{d}{dt}#1\|}
\newcommand*\ap[2]{\tilde{#1}_{#2}}
\newcommand*\F[0]{\mathcal{F}}
\newcommand*\D[0]{\mathcal{D}}
\renewcommand*\H[0]{\mathcal{H}}
% \newcommand*\G[0]{\mathcal{G}}
\newcommand*\Pspace[0]{\mathscr{P}}
\newcommand*\Uspace[0]{\mathbb{U}}
\renewcommand*\t[1]{\tilde{#1}}
\renewcommand*\d[0]{\delta}
\newcommand*\ot[1]{#1^{\perp}}
\newcommand*\proj[0]{\text{Proj}}
%
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand*\lrb[1]{\left[#1\right]}
\newcommand*\lrbb[1]{\left\{#1\right\}}
\newcommand*\lrp[1]{\left(#1\right)}
\newcommand*\lrn[1]{\left\|#1\right\|}
\newcommand*\lrw[1]{\left\langle#1\right\rangle}
\newcommand*\eu[1]{\left\| #1\right\|}
\newcommand*\xt[0]{\tilde{x}}
% \newcommand*\vt[0]{\tilde{v}}
\newcommand*\pt[0]{\tilde{p}}
\newcommand*\A[0]{\mathcal{A}}
\newcommand*\B[0]{\mathcal{B}}
\newcommand*\cvec[2]{\begin{bmatrix} #1\\#2\end{bmatrix}}
\newcommand*\bmat[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand*\pa[0]{\phi^\mathcal{A}}
\newcommand*\pb[0]{\phi^\mathcal{B}}
\newcommand*\Ts[0]{{T_{sync}}}
\newcommand*\tm[0]{{t^-}}
\newcommand*\ind[1]{{\mathds{1}\lrbb{#1}}}
\renewcommand*\proj[2]{{\Pi_{#1}\lrp{#2}}}
\renewcommand*{\tt}{{\tau(t)}}
\newcommand*{\ttm}{{\tau(\tm)}}
%
\renewcommand*{\Re}{\mathbb{R}}
\renewcommand*{\P}{\mathbf{P}}
\newcommand{\blank}[1]{\hfil\penalty1000\hfilneg\rule[-3pt]{#1}{0.4pt}} %
%
%
%
%
\def\mI{\mathrm{I}}

\def\vtheta{{{ \theta}}}
\def\dtheta{\Delta_\vtheta}
\def\vTheta{{{\Theta}}}
%
\def\vzeta{{{\zeta}}}
\def\vx{{\bf x}}
%
\def\vX{\Theta}
\def\vy{{\bf y}}
\def\vz{{\bf z}}
\def\vv{{\bf v}}
\def\rd{\mathrm{d}}
\def\rT{{\rm T}}
\def\ball{\mathbb{B}}
\def\mI{\mathrm{I}}

%
% \newcommand{\1}{\ensuremath{{\sf (i)}}}
% \newcommand{\2}{\ensuremath{{\sf (ii)}}}
% \newcommand{\3}{\ensuremath{{\sf (iii)}}}
% \newcommand{\4}{\ensuremath{{\sf (iv)}}}
% \newcommand{\5}{\ensuremath{{\sf (v)}}}
% \newcommand{\6}{\ensuremath{{\sf (vi)}}}
% \newcommand{\7}{\ensuremath{{\sf (vii)}}}
% \newcommand{\8}{\ensuremath{{\sf (viii)}}}


%

%
\newcommand*{\Q}{\mathbf{Q}}
\newcommand*{\transpose}{\rm{T}}
\newcommand{\stepsize}{\eta}

\newcommand{\mixingerror}{\epsilon}
\newcommand{\mixingtime}{\tau_{\text{mix}}}

\newcommand{\hmu}{\widehat{\mu}}

\newcommand{\targetmeasure}{\mu}
\newcommand{\stationary}{\ensuremath{\Pi}}
\newcommand{\warmparam}{\beta}
\newcommand{\func}{U}
%
\newcommand{\proposal}{\mathcal{P}}


\newcommand{\step}{h}
\newcommand{\stepfunc}{w}
\newcommand{\stepbound}{\tilde{w}}
\newcommand{\scalar}{\alpha}
\newcommand{\tvscalar}{\gamma}


\newcommand{\transition}{\mathcal{T}}

\newcommand{\tagula}{\text{\tiny ULA}}
\newcommand{\tagmala}{\text{\tiny MALA}}
\newcommand{\tagmrw}{\text{\tiny MRW}}

\newcommand{\flow}{\phi}
\newcommand{\conductance}{\Phi}

\newcommand{\radius}{r}
\newcommand{\truncball}{\mathcal{R}}
\newcommand{\maxgrad}{\mathcal{D}}

\newcommand{\convexset}{\ensuremath{\mathcal{K}}}

\newcommand{\scparam}{m}
\newcommand{\smoothness}{L}
\newcommand{\condition}{\ensuremath{\kappa}}

\newcommand{\dims}{d}
\newcommand{\obs}{n}
\newcommand{\mydefn}{:=}
\newcommand{\logsobconstU}{\rho_U}
\newcommand{\logsobconst}{\rho}
\newcommand{\discretized}{\tilde}

\newcommand{\inprod}[2]{\ensuremath{\left\langle #1 , \, #2 \right\rangle}}
%
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
%
\newcommand{\Exs}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}

%
%
%
%
\newcommand{\kldiv}{\text{KL}\infdivx}

\newcommand{\MIS}{\mathrm{MIS}}


\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{Ber}}}

\newcommand{\Ot}{\tilde{\mathcal{O}}}
\newcommand{\Pc}{P}
\newcommand{\Pa}{Q}
%
\newcommand{\sphere}{\mathbb{S}}

%
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\left\| #1\right\|_{#2}}

\newcommand{\hessianlip}{L_2}
%
\newcommand{\param}{\theta}
\newcommand{\Param}{\Theta}
\newcommand{\paramb}{\nu}
\newcommand{\data}{\mathcal{D}}
\newcommand{\z}{z}
\newcommand{\x}{x}
\newcommand{\prior}{p_\param}
\newcommand{\hyper}{\alpha}
\newcommand{\tfunc}{h}
\newcommand{\pmean}{q}
\newcommand{\f}{f}
\newcommand{\stp}{\eta}
\newcommand{\grad}{\nabla}
\newcommand{\gnoise}{\xi}
\newcommand{\lang}{\theta}
\newcommand{\g}{g}
\newcommand{\Cr}{C_{R}}
\newcommand{\Csa}{C_{\small{\Sigma, 1}}}
\newcommand{\Csb}{C_{\small{\Sigma, 2}}}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}


% \DeclareMathOperator*{\argmax}{argmax}
\newtheorem{theorem2}{Theorem}[section]
\usepackage{multirow}
\usepackage{caption}
\usepackage{subcaption} \newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\mb}{\mathbb}
\newcommand{\mc}{\mathcal}
\newcommand{\rar}{\rightarrow}
\newcommand{\ts}{\textsuperscript}
\DeclareMathOperator*{\argmin}{argmin}

\newcommand{\M}[1]{{\mathbf{#1}}} % matrix
\newcommand{\T}[1]{{\mathcal{#1}}} % tensor
\newcommand{\V}[1]{{\mathbf{#1}}} % vector

\newcommand{\xmark}{$\times$}%


==> sections/app.tex <==
\section{Climate Model for Temperature}
\label{Appendix:climate}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{fig/fig4.png}
    \caption{Left: Region of interest \citep{wiki_peru}. Upper Right: sample from low-fidelity temperature model. Lower Right: sample from high-fidelity temperature model.}
    \label{fig:peru}
\end{figure}

\section{Neural Processs Baselines}
\label{Appendix:np_baseline}
\subsection{Single-Fidelity Neural Processes (SF-NP).}
A simple way to apply NP to the multi-fidelity problem is to train NP only using the data at high fidelity level only assuming it is not correlated with the data at the low fidelity level. We name it as Single-Fidelity Neural Processes baseline (SF-NP). During the training process, the high level training data can be randomly split into context set $\mathcal{D}^c_h$ and target set $\mathcal{D}^t_h$. We use the corresponding evidence lower bound (ELBO) as the training loss function:

% \begin{align}
% \begin{split}
%     & \log p(y^h_t|x^h_t,x^h_c,y^h_c,\theta) \geq\\ 
%     & \mathbb{E}_{q_\phi(z|x^h_c,y^h_c,x^h_t,y^h_t)} \big[  \log p(y^h_t|z, x^h_t,\theta)\big] - \\
%     & \text{KL}\big( q_\phi(z| x^h_c,y^h_c)\| q_\phi(z|x^h_c,y^h_c,x^h_t,y^h_t ) \big)
%     \label{eqn:sfnp}
% \end{split}
% \end{align}

\begin{align}
\begin{split}
    & \log p(y^t_{h,1:M}|x^t_{h,1:M},\mathcal{D}^c_h,\theta) \geq\\ 
    & \mathbb{E}_{q_\phi(z|\mathcal{D}^c_h \cup \mathcal{D}^t_h)} \big[ \sum_{m=1}^M\log p(y^t_{h,m}|z, x^t_{h,m},\theta)+log\frac{q_\phi(z|\mathcal{D}^c_h)}{q_\phi(z|\mathcal{D}^c_h \cup \mathcal{D}^t_h)}\big]\\
    \label{eqn:elbo_sfnp}
\end{split}
\end{align}

where $p(\theta)$ is a decoder in a neural network and $q_\phi$ indicates a encoder to inference the latent variable $z$.

% \allen{how to generate predictions, conditioned on training set}

\subsection{Multi-Fidelity Neural Processes (MF-NP).} 
%
Multi-Fidelity Neural Processes (MF-NP) \cite{wang2020mfpc} assume a comprehensive correlation between multi-fidelity models $y_h$ and $y_l$ can be represented as:
\begin{align}
\begin{split}
    y_h(x) = \mathcal{G}(y_l(x)) + \delta(x),
    \label{eqn:mfnp_gen}
\end{split}
\end{align}
where $\mathcal{G}$ is a nonlinear function mapping the low fidelity data to high fidelity data, and $\delta(x)$ is space dependent bias between fidelity levels.
To train MF-NP model, we take data pairs $(x,y_l(x))$ as the input to predict the corresponding $y_h(x)$. The corresponding context sets $\mathcal{D}_l^c \equiv \{x^c_{h,n},{y^c_{l,n}}, {y^c_{h,n}}\}_{n=1}^{N_l}$ and target sets $\mathcal{D}_l^t \equiv \{x^t_{h,m},{y^t_{l,m}},{y^t_{h,n}}\}_{m=1}^{M_l}$. The ELBO for the training process is:

% \begin{align}
% \begin{split}
%     &\log p(y^h_t|x^h_t,y^l_t,x^h_c,y^l_c,y^h_c,\theta) \geq\\ &\mathbb{E}_{q(z|x^h_c,y^l_c,y^h_c,x^h_t,y^l_t,y^h_t)} \big[
%     \log p(y^h_t|z, x^h_t, y^l_t, \theta)\big] - \\
%     & \text{KL}\big( q_\phi(z| x^h_c,y^l_c,y^h_c)\| q_\phi(z|x^h_c,y^l_c,y^h_c,x^h_t,y^l_t,y^h_t) \big)
%     \label{eqn:mfnp}
% \end{split}
% \end{align}

\begin{align}
\begin{split}
    & \log p(y^t_{h,1:M}|x^t_{h,1:M},y^t_{l,1:M},\mathcal{D}^c_h,\theta) \geq\\ 
    & \mathbb{E}_{q_\phi(z|\mathcal{D}^c_h \cup \mathcal{D}^t_h)} \big[ \sum_{m=1}^M\log p(y^t_{h,m}|z, x^t_{h,m},y^t_{l,m},\theta)+log\frac{q_\phi(z|\mathcal{D}^c_h)}{q_\phi(z|\mathcal{D}^c_h \cup \mathcal{D}^t_h)}\big]\\
    \label{eqn:elbo_mfnp}
\end{split}
\end{align}

Since this method requires $(x,y_l(x),y_h(x))$ for input and output, it can not fully utilize the training data at the low fidelity level which $y_h(x)$ is unknown.  Furthermore, MF-NP requires a nested data structure, which means the training inputs of the high fidelity level need to be a subset of the training inputs of the low fidelity level. On the contrary, if  the training inputs at the different fidelity level are disjoint, no data set can be used for training.

% there will be an empty training set for the MF-NP model.
% which causes the key limitation of this method.

% We could also view MF-NP as a NP version of nonlinear autoregressive multi-fidelity GP regression model (NARGP) assuming $y^l(x)$ is available for $x$ in the test set. 


